High Speed Peltier Calorimeter for the Calibration of High Bandwidth Power Measurement Equipment

Accurate power measurements of electronic components operating at high frequencies are vital in determining where power losses occur in a system such as a power converter. Such power measurements must be carried out with equipment that can accurately measure real power at high frequency. We present the design of a high speed calorimeter to address this requirement, capable of reaching a steady state in less than 10 minutes. The system uses Peltier thermoelectric coolers to remove heat generated in a load resistance, and was calibrated against known real power measurements using an artificial neural network. A dead zone controller was used to achieve stable power measurements. The calibration was validated and shown to have an absolute accuracy of +/-8 mW (95% confidence interval) for measurements of real power from 0.1 to 5 W.

==> CalorimeterPaper/05_ElectricalDesign.tex <==
\section{Electrical Design}

\hl{Discuss the electrical design. Why the peltiers are controlled with analog. Temperature sensing, etc.}
